Large deviations for quasi-periodic cocycles with singularities

We derive large deviations type (LDT) estimates for linear cocycles over an ergodic multifrequency torus translation. These models are called quasi-periodic cocycles. We make the following assumptions on the model: the translation vector satisfies a generic Diophantine condition, and the fiber action is given by a matrix valued analytic function of several variables which is not identically singular. The LDT estimates obtained here depend on some uniform measurements on the cocycle. Our general results derived in [9] regarding the continuity properties of the Lyapunov exponents (LE) and of the Oseledets filtration and decompositions are then applicable, and we obtain local weak-Holder continuity of these quantities in the presence of gaps in the Lyapunov spectrum. The main new feature of this work is allowing a cocycle depending on several variables to have singularities, i.e. points of non invertibility. This requires a careful analysis of the set of zeros of certain analytic functions of several variables and of the singularities (i.e. negative infinity values) of pluri-subharmonic functions related to the iterates of the cocycle. A refinement of this method in the one variable case leads to a stronger LDT estimate and in turn to a stronger, nearly-Holder modulus of continuity of the LE, Oseledets filtration and Oseledets decomposition. This is a draft of a chapter in our forthcoming research monograph [9].

==> recycle.tex <==
We now state and prove the splitting lemma in $d=2$ variables. A similar statement and argument applies to any number of variables. 



\begin{lemma}\label{splitting-lemma-2var}
Let $u (z)$ be a pluri subharmonic function in a neighborhood of  $\strip_r^2$, satisfying the bounds:
\begin{align}
& u (z)   \le  C_1   &\text{for all } z \in \strip_r^2 \label{sl-2var-h1}\\
& \norml{u (\cdot, x_2)}{\Lpx{2}{x_1}}   \le C_2   &\text{for all } x_2 \notin \B \label{sl-2var-h2} \\
& \norml{u (x_1, \cdot)}{\Lpx{2}{x_2}}  \le C_2    &\text{for all } x_1 \notin \B \label{sl-2var-h3} \\
& \norml{u}{L^2(\T^2)}   \le C_2 \label{sl-2var-h4}
\end{align}
where $\B \subset \T$. 

Let $C := C_1 + C_2$ be the 'total Riesz weight' of $u$. 
If $u (x)$ satisfies the weak a-priori estimate:
\begin{equation}\label{sl-2var-weak}
\abs{ \{ x \in \T^2 \colon \abs{ u (x) - \avg{u} }  > \ep_0 \} } < \ep_1
\end{equation} 
with $\ep_1 \le \ep_0^8$, then
\begin{equation}\label{sl-2var-strong}
\abs{ \{ x \in \T^2  \colon \abs{ u (x) - \avg{u} }  > \ep_0^{1/4} \} } < e^{- c \, \ep_0^{- 1/4}} + \abs{\B}
\end{equation} 
where $c \sim \bigl(\frac{C}{r}\bigr)^{- 5/4}$

For $d$ variables, replace the powers $1/4$ by $1/2 d$ etc. 
\end{lemma}

\begin{remark}\rm{
This type of estimate is available (see Lemma 4.12 in \cite{B}) for {\em bounded} pluri subharmonic functions. We show that the result also holds under weaker assumptions, namely an upper bound,  a global $L^2$ bound and uniform separately  $L^2$ - bounds along horizontal and vertical lines (or hyperplanes for more variables). We do not require here that these bounds hold for all such lines. 

As explained in Remark~\ref{to-change-or-not-to-change-vars}, in applications to iterates of a cocycle, this will not {\em a-priori} hold for all lines, but for 'many' such lines. Moreover, these bounds will depend polynomially on the number of iterates.

Alternatively (and this is the path we have  chosen here), these separately $L^2$-bounds will indeed hold uniformly and along all such lines, but only {\em after a change of variables}.
}
\end{remark}

\begin{proof}
Clearly $\abs{\avg{u}} \le C_2$, so replacing $u$ by $u - \avg{u}$ will only at most double the total Riesz weight. Hence we may assume, that being the case for $u - \avg{u}$, that $\avg{u} = 0$. 

Let $\Bt$ be the set in \eqref{sl-2var-weak}, so $\abs{\Bt} < \ep_1$ and split $u = u_0 + u_1$, where $u_0 := u \cdot \ind_{\Bt^{\comp}}$ and $u_1 := u \cdot \ind_{\Bt}$. Then as before, 
$\norml{u_0}{L^{\infty} (\T^2)} \le \ep_0$ and $\norml{u_1}{L^1 (\T^2)} \le C_2 \, \ep_1^{1/2}$.

We will apply the one-variable result Lemma~\ref{decay-BMO-1var} to $x_1 \mapsto u (x_1, x_2)$ for $x_2$ outside a small set.

Let 
$$\B_2 := \{ x_2 \in \T \colon \int_\T \abs{ u_1 (x_1, x_2) } d x_1 \ge \ep_1^{1/4} \}$$
Then by Chebyshev's inequality $\abs{\B_2} \leq \epsilon_1^{-1/4}\norml{u_1}{L^1 (\T^2)} \leq  C_2 \, \ep_1^{1/4}$.
%Then $\abs{\B_2} < C_2 \, \ep_1^{1/4}$, for if we denote
%$$\phi (x_2) := \int_\T  \abs{ u_1 (x_1, x_2) } d x_1 \, ( \ge 0)$$
%then
%$$\abs{\B_2} \ep_1^{1/4} \le \int_{\B_2} \phi (x_2) d x_2 \le \int_\T \phi (x_2) d x_2 = \norml{u_1}{L^1 (\T^2)} < C_2  \ep_1^{1/2}$$


Let $\Bbar_2 := \B_2 \cup \B$. We may of course assume that $\abs{\B} < C_2 \, \ep_1^{1/4}$, since otherwise \eqref{sl-2var-weak} is stronger than \eqref{sl-2var-strong}. Therefore, $\abs{\Bbar_2} \less C_2 \ep_1^{1/4}$.

For every $x_2 \notin \Bbar_2$, we can apply Lemma~\ref{decay-BMO-1var} to the one variable function $v (z_1) := u (z_1, x_2)$.

Indeed, write $v (x_1) = v_0 (x_1) + v_1 (x_1)$, where $v_0 (x_1) := u_0 (x_1, x_2)$, $v_1 (x_1) := u_1 (x_1, x_2)$. Then clearly
\begin{align*}
& v (z_1)  \le C_1    & \text{for all } z_1 \in \strip_r \\
& \norml{v}{\Lp{2}}  = \norml{u (\cdot, x_2)}{\Lpx{2}{x_1}} \le C_2   & \text{since } x_2 \notin \B \\
& \norml{v_0}{\Lp{\infty}}  \le \norml{u_0}{L^{\infty} (\T^2)} \le \ep_0  \\
& \norml{v_1}{\Lp{1}} = \int_\T \abs{ u_1 (x_1, x_2)} d x_1 < \ep_1^{1/4}   & \text{since } x_2 \notin \B_2
\end{align*}


Since $\ep_1 \le \ep_0^8$, 
Lemma~\ref{decay-BMO-1var} then implies:
$$\norml{u (\cdot, x_2)}{BMO_{x_1} (\T)} = \norml{v}{BMO (\T)} \less \ep_0 + \bigl( \ep_1^{1/4} \, C / r \bigr)^{1/2} \less (C/r)^{1/2} \, \ep_0\;. $$

By John-Nirenberg inequality, BMO functions are exponentially integrable, so for an absolute constant $c_0 > 0$ and for all $x_2 \notin \Bbar_2$ 
$$\int_\T e^{ c_0 \frac{\sabs{u (x_1, x_2)}}{(C/r)^{1/2} \, \ep_0} } \ d x_1 \leq  \int_\T e^{ c_0 \frac{\sabs{u (x_1, x_2)}}{\norml{u (\cdot, x_2)}{BMO_{x_1} (\T)} } } \ d x_1  
\less 1$$

Integrating in $x_2 \in \Bbar_2^{\comp}$ we then have:
\begin{equation}\label{sl-2var-p1}
\int_{\Bbar_2^{\comp}}   \int_\T e^{ c_0 \frac{\sabs{u (x_1, x_2)}}{(C/r)^{1/2} \, \ep_0} } \, d x_1 d x_2 \less 1\;.
\end{equation}

We will again apply the one-variable BMO estimate, this time to $x_2 \mapsto u (x_1, x_2)$, for $x_1$ outside an exponentially small set.

Denote
$$\delta_0 := e^{- c_0 \, (C/r)^{-1/2} \, \ep_0^{-1/2}}\;, $$
consider the function
$$\phi(x_1,x_2) :=  e^{ c_0 \,\frac{ \sabs{ u (x_1, x_2) } }{ (C/r)^{1/2}\, \ep_0} }\;, $$

and let

$$\B_1 := \{ x_1 \in \T \colon \int_{\Bbar_2^{\comp}}   \phi(x_1,x_2)\,dx_2  > \delta_0^{-1} \}\;. $$
%$$\B_1 := \{ x_1 \in \T \colon \int_{\Bbar_2^{\comp}}   e^{c_0 \, (C/r)^{-1/2} \, \ep_0^{-1} \, \sabs{ u (x_1, x_2) }} \, d x_2 > \delta_0^{-1} \}\;. $$


Then  by Chebyshev's inequality
$\abs{\B_1} \less \delta_0$. 
%, for if we denote 
%$$\phi (x_1) := \int_{\Bbar_2^{\comp}}   e^{- c_0 \, (C/r)^{-1/2} \, \ep_0^{-1} \, \sabs{ u (x_1, x_2) }} \, d x_2 \ (\ge 0)$$
%then from the definition of $\B_1$ and from \eqref{sl-2var-p1} we have:
%$$\abs{\B_1} \cdot \delta_0^{-1} \le \int_{\B_1} \phi (x_1) d x_1 \le \int_\T \phi (x_1) d x_1 \less 1$$
%

Let $\Bbar_1 := \B_1 \cup \B$, so $\abs{\Bbar_1} < \delta_0 + \abs{\B}$.

Fix $x_1 \notin \Bbar_1$ and define the slice
$$\B^*_2 (x_1) := \{ x_2 \in \T \colon \abs{u (x_1, x_2)} > 2 \ep_0^{1/2} \}$$

We estimate the measure of the set 
$$\B^*_2 (x_1) = (\B^*_2 (x_1) \cap \Bbar_2^{\comp} ) \cup (\B^*_2 (x_1) \cap \Bbar_2)\;. $$ 
Remark that $\abs{ u (x_1, x_2) } > 2 \ep_0^{1/2}$  if and only if
$\phi(x_1,x_2)\geq \delta_0^{-2}$.
Since for $x_2 \in \B^*_2 (x_1)$, $\abs{ u (x_1, x_2) } > 2 \ep_0^{1/2}$, by Chebyshev's inequality, applied to $\phi_{x_1}=\phi(x_1,\cdot):\Bbar_2^{\comp}\to\R$ we have:
\begin{align*}
\abs{ \B^*_2 (x_1) \cap \Bbar_2^{\comp} } \leq
\delta_0^2\int_{\Bbar_2^{\comp} }  \phi(x_1,x_2)\,dx_2 \leq \delta_0\;. 
\end{align*} 
% we have:
%\begin{align}
%\int_{\B^*_2 (x_1) \cap \Bbar_2^{\comp}}   e^{c_0 \, (C/r)^{-1/2} \, \ep_0^{-1} \, \sabs{ u (x_1, x_2) }} \, d x_1 
%& \ge e^{c_0 \, (C/r)^{-1/2} \, 2 \ep_0^{-1/2}}  \cdot \abs{ \B^*_2 (x_1) \cap \Bbar_2^{\comp}}  \notag \\
%& = \delta_0^{- 2} \, \abs{ \B^*_2 (x_1) \cap \Bbar_2^{\comp} }
%\label{sl-2var-p2}
%\end{align}
%
%
%Moreover, since $x_1 \notin \Bbar_1$, we have 
%\begin{equation} \label{sl-2var-p3}
%\int_{\B^*_2 (x_1) \cap \Bbar_2^{\comp}}   e^{c_0 \, (C/r)^{-1/2} \, \ep_0^{-1} \, \sabs{ u (x_1, x_2) }} \, d x_1 
% \le  \int_{\Bbar_2^{\comp}}   e^{c_0 \, (C/r)^{-1/2} \, \ep_0^{-1} \, \sabs{ u (x_1, x_2) }} \, d x_1  \le \delta_0^{-1}  
%\end{equation}
%
%From \eqref{sl-2var-p2} and \eqref{sl-2var-p3} we obtain: $\abs{ \B^*_2 (x_1) \cap \Bbar_2^{\comp}  } < \delta_0$.
%

Furthemore,
$$\abs{ \B^*_2 (x_1) \cap \Bbar_2 } \le \abs{ \Bbar_2 } < C_2 \, \ep_1^{1/4}$$

We may assume that $\delta_0 = e^{- c_0 \, (C/r)^{-1/2} \, \ep_0^{-1/2}} < C_2 \, \ep_1^{1/4}$, since otherwise \eqref{sl-2var-weak} is stronger than \eqref{sl-2var-strong}. 

Therefore, if $x_1 \notin \Bbar_1$, then $\abs{\B^*_2 (x_1) } \less C_2 \, \ep_1^{1/4}$.

Fix $x_1 \notin \Bbar_1$, let $v (z_2) := u (x_1, z_2)$ and write $v (x_2) = v_0 (x_2) + v_1 (x_2)$, where $v_0 (x_2) := v (x_2) \cdot \ind_{\B^*_2 (x_1)^{\comp}}$ and 
$v_1 (x_2) := v (x_2) \cdot \ind_{\B^*_2 (x_1)}$.

Then clearly
\begin{align*}
& v (z_2)   \le C_1  \quad \text{ for all } z_2 \in \strip_r \,, \\
& \norml{v}{\Lp{2}}   = \norml{u (x_1, \cdot)}{\Lpx{2}{x_2}} \le C_2   \; \text{ since } x_1 \notin \B \,, \\
& \norml{v_0}{\Lp{\infty}}   \less 2 \ep_0^{1/2} \;  \text{ by the definitions of } v_0 \text{ and }  \B^*_2 (x_1)  \,, \\
& \norml{v_1}{\Lp{1}}  \le \norml{v}{\Lp{2}} \cdot \norml{\ind_{\B^*_2 (x_1)}}{\Lp{2}} \;, \\
& \qquad \qquad=  \norml{u (x_1, \cdot)}{\Lpx{2}{x_2}} \cdot \abs{\B^*_2 (x_1)}^{1/2} \le C_2 \, (C_2 \, \ep_1^{1/4})^{1/2} \le C_2^{3/2} \ep_0\;.
\end{align*}


Lemma~\ref{decay-BMO-1var} implies:
$$\norml{v}{BMO (\T)} \less 2 \ep_0^{1/2} + (C_2^{3/2} \ep_0 \, C / r)^{1/2} \less (C/r)^{5/4} \ep_0^{1/2}$$

Applying John-Nirenberg inequality to $v (x_2)$ we have:   if $x_1 \notin \Bbar_1$ then:
\begin{align}\label{sl-2var-p5}
\abs{ \{  x_2 \in \T \colon \abs{u (x_1, x_2) } > \ep_0^{1/4}  \} } = \abs{ \{  x_2 \in \T \colon \abs{v (x_2) } > \ep_0^{1/4}  \} } \notag\\
\le e^{- c_0 \, \ep_0^{1/4} / \norml{v}{BMO(\T)}} \le e^{- c_0 \, (C/r)^{-5/4} \, \ep_0^{-1/4} }
\end{align}

We conclude:
\begin{align*}
& \{ (x_1, x_2) \in \T^2 \colon \abs{ u (x_1, x_2) } > \ep_0^{1/4}  \} \\
& \subset (\Bbar_1 \times \T) 
 \cup \{ (x_1, x_2) \colon x_1 \notin \Bbar_1 \text{ and } \abs{ u (x_1, x_2) } > \ep_0^{1/4}  \} 
\end{align*}

But
$$\abs{\Bbar_1 \times \T} = \abs{\Bbar_1} < \delta_0 + \abs{\B} =  e^{- c_0 \, (C/r)^{-1/2} \, \ep_0^{-1/2}} + \abs{\B} $$
while by \eqref{sl-2var-p5} and Fubini
$$ \{ (x_1, x_2) \colon x_1 \notin \Bbar_1 \text{ and } \abs{ u (x_1, x_2) } > \ep_0^{1/4}  \}  < e^{- c_0 \, (C/r)^{-5/4} \, \ep_0^{-1/4}} 
$$
which concludes the proof.
\end{proof}

















